A O(1/eps^2)^n Time Sieving Algorithm for Approximate Integer Programming

The Integer Programming Problem (IP) for a polytope P \subseteq R^n is to find an integer point in P or decide that P is integer free. We give an algorithm for an approximate version of this problem, which correctly decides whether P contains an integer point or whether a (1+\eps) scaling of P around its barycenter is integer free in time O(1/\eps^2)^n. We reduce this approximate IP question to an approximate Closest Vector Problem (CVP) in a "near-symmetric" semi-norm, which we solve via a sieving technique first developed by Ajtai, Kumar, and Sivakumar (STOC 2001). Our main technical contribution is an extension of the AKS sieving technique which works for any near-symmetric semi-norm. Our results also extend to general convex bodies and lattices.

==> analysis.tex <==
\section{Algorithm Analysis}
\label{sec:alg-analysis}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "faster-ip"
%%% End: 

